KoLA: Carefully Benchmarking World Knowledge of Large Language Models

The unprecedented performance of large language models (LLMs) necessitates improvements in evaluations. Rather than merely exploring the breadth of LLM abilities, we believe meticulous and thoughtful designs are essential to thorough, unbiased, and applicable evaluations. Given the importance of world knowledge to LLMs, we construct a Knowledge-oriented LLM Assessment benchmark (KoLA), in which we carefully design three crucial factors: (1) For \textbf{ability modeling}, we mimic human cognition to form a four-level taxonomy of knowledge-related abilities, covering $19$ tasks. (2) For \textbf{data}, to ensure fair comparisons, we use both Wikipedia, a corpus prevalently pre-trained by LLMs, along with continuously collected emerging corpora, aiming to evaluate the capacity to handle unseen data and evolving knowledge. (3) For \textbf{evaluation criteria}, we adopt a contrastive system, including overall standard scores for better numerical comparability across tasks and models and a unique self-contrast metric for automatically evaluating knowledge-creating ability. We evaluate $28$ open-source and commercial LLMs and obtain some intriguing findings. The KoLA dataset and open-participation leaderboard are publicly released at https://kola.xlore.cn and will be continuously updated to provide references for developing LLMs and knowledge-related systems.

==> Table/raw_score_level1_2.tex <==
\begin{table}[ht]
\caption{Raw performance of Knowledge Memorization and Understanding Level.}
\label{tab:raw_level1-2}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l|llll|lllllllll@{}}
\toprule
\multirow{2}{*}{\textbf{Model}}    & \multicolumn{4}{c}{\textbf{Level 1: KM}} & \multicolumn{9}{|c}{\textbf{Level 2: KU}}                     \\ \cmidrule(l){2-14} 
                         & \textbf{1-1}    & \textbf{1-2}   & \textbf{1-3}   & \textbf{Rank}   & \textbf{2-1} & \textbf{2-2} & \textbf{2-3} & \textbf{2-4} & \textbf{2-5} & \textbf{2-6} & \textbf{2-7} & \textbf{2-8} & \textbf{Rank} \\ \midrule
FLAN-T5-XXL              & 20.09  &   17.74 &       &        &     &     &     &     &     &     &     &     &      \\
UL2                      & 4.88   &  5.12   &       &        &     &     &     &     &     &     &     &     &      \\
FLAN-UL2                 & 18.5   & 13.24       &        &     &     &     &     &     &     &     &     &      \\
GPT-JT (6B)              &  1.75 &  1.30   &        &        &     &     &     &     &     &     &     &     &      \\
GPT-J (6B)               &    2.26 &  1.21  &       &        &     &     &     &     &     &     &     &     &      \\
GPT-NeoX (20B)           & 1.78 & 2.18    &       &        &     &     &     &     &     &     &     &     &      \\
BLOOM (7B)               & 2.33  &  2.81   &       &        &     &     &     &     &     &     &     &     &      \\
T0++                     &  12.89  & 11.14   &       &        &     &     &     &     &     &     &     &     &      \\
LLaMa                    & 3.97 &  4.67    &       &        &     &     &     &     &     &     &     &     &      \\
Alpaca                   & 2.58   & 4.49        &       &        &     &     &     &     &     &     &     &     &      \\
J2-Jumbo-Instruct        &  8.21  & 8.77       &       &        &     &     &     &     &     &     &     &     &      \\
Cohere-command           &  21.53  & 19.26      &       &        &     &     &     &     &     &     &     &     &      \\
GPT-3.5-turbo            &  18.74  & 22.08        &       &        &     &     &     &     &     &     &     &     &      \\
GPT-3\_curie\_v1         &  0.41 & 0.67          &       &        &     &     &     &     &     &     &     &     &      \\
GPT3\_davinci\_v1        & 0.89  &  0.78         &       &        &     &     &     &     &     &     &     &     &      \\
instructGPT\_curie\_v1   &  5.93 & 13.88        &       &        &     &     &     &     &     &     &     &     &      \\
InstructGPT\_davinci\_v2 & 12.58   & 16.20        &       &        &     &     &     &     &     &     &     &     &      \\
GLM-130B                 & 2.78  &  4.41        &       &        &     &     &     &     &     &     &     &     &      \\
GPT4                     & 24.21  & 26.54       &       &        &     &     &     &     &     &     &     &     &      \\
ChatGLM-130B             & 10.93  &  20.30       &       &        &     &     &     &     &     &     &     &     &      \\ 
\midrule
average  score        & 8.86  &  9.84      &       &        &     &     &     &     &     &     &     &     &      \\ 
standard deviation             & 7.73  &  8.03       &       &        &     &     &     &     &     &     &     &     &      \\ 
\bottomrule
\end{tabular}}
\end{table}




\begin{table}[ht]
\caption{Raw performance of Knowledge Applying and Creating Level.}
\label{tab:raw_level3-4}
\centering
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{@{}l|lllllll|lll@{}}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{7}{c}{\textbf{Level 3: KA}}                                                                                                                                                                                                            & \multicolumn{3}{|c}{\textbf{Level 4: KC}}                                                                \\ \cmidrule(l){2-11} 
                                & \multicolumn{1}{c}{\textbf{3-1}} & \multicolumn{1}{c}{\textbf{3-2}} & \multicolumn{1}{c}{\textbf{3-3}} & \multicolumn{1}{c}{\textbf{3-4}} & \multicolumn{1}{c}{\textbf{3-5}} & \multicolumn{1}{c}{\textbf{3-6}} & \multicolumn{1}{c}{\textbf{Rank}} & \multicolumn{1}{|c}{\textbf{4-1}} & \multicolumn{1}{c}{\textbf{4-2}} & \multicolumn{1}{c}{\textbf{Rank}} \\ \midrule
FLAN-T5-XXL                     &        23.7                      &    35.30                              &     7.50                             &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
UL2                             &        6.00                      &    15.80                              &   3.90                               &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
FLAN-UL2                        &       27.10                      &   34.00                               &   10.60                              &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
GPT-JT (6B)                     &       13.80                      &  25.50                                &    2.80                              &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
GPT-J (6B)                      &    19.20                         &  26.60                                &   4.60                               &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
GPT-NeoX (20B)                  &  1.00                            &  3.60                                 &  0.00                                &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
BLOOM (7B)                      &   4.40                           &   11.40                               &  0.00                                &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
T0++                            &   7.20                           &   11.80                               &   3.20                               &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
LLaMa                           &   2.80                           &    23.00                              &   11.70                              &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
Alpaca                          &      1.80                        &   8.40                                &   1.80                               &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
J2-Jumbo-Instruct               &    23.90                         &   19.60                               &   6.90                               &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
Cohere-command                  &   17.30                          &  28.70                                &   13.40                              &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
GPT-3.5-turbo                   &    33.60                         &  29.50                                &  17.50                               &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
GPT-3\_curie\_v1                &    7.30                          &  4.70                                 &   1.60                               &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
GPT3\_davinci\_v1               &      4.20                        &   3.20                                &  2.70                                &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
instructGPT\_curie\_v1          &     13.90                        &   24.60                               &  3.40                                &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
InstructGPT\_davinci\_v2        &   13.20                          &    26.90                              &      12.90                           &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
GLM-130B                        &   8.00                           &   2.70                                &     0.60                             &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
GPT4                            &    34.60                         &    45.90                              &     28.40                            &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\
ChatGLM                         &    17.40                         &    21.80                              &    5.20                              &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\ 
\midrule
average  score          &    14.02               &             20.15                     &           6.93                   &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\ 
standard deviation      &    10.11               &            11.83                      &       6.92                       &                                  &                                  &                                  &                                   &                                  &                                  &                                   \\ 
\bottomrule
\end{tabular}}
\end{table}

